LangGas: Introducing Language in Selective Zero-Shot Background Subtraction for Semi-Transparent Gas Leak Detection with a New Dataset

Gas leakage poses a significant hazard that requires prevention. Traditionally, human inspection has been used for detection, a slow and labour-intensive process. Recent research has applied machine learning techniques to this problem, yet there remains a shortage of high-quality, publicly available datasets. This paper introduces a synthetic dataset, SimGas, featuring diverse backgrounds, interfering foreground objects, diverse leak locations, and precise segmentation ground truth. We propose a zero-shot method that combines background subtraction, zero-shot object detection, filtering, and segmentation to leverage this dataset. Experimental results indicate that our approach significantly outperforms baseline methods based solely on background subtraction and zero-shot object detection with segmentation, reaching an IoU of 69%. We also present an analysis of various prompt configurations and threshold settings to provide deeper insights into the performance of our method. Finally, we qualitatively (because of the lack of ground truth) tested our performance on GasVid and reached decent results on the real-world dataset. The dataset, code, and full qualitative results are available at https://github.com/weathon/Lang-Gas.

==> sec/trash.tex <==

We also examined the frequency of these keywords in the model's training dataset. However, since the training data for Owl-v2 \cite{owlv2}, WebLI \cite{webli} is not publicly available, we analyzed another publicly available image-text dataset, CC12M \cite{changpinyo2021cc12m}, which was used in training Owl-ViT \cite{owlvit}—the model that generated pseudo-labels for Owl-v2 \cite{owlv2}.

Using regular expressions, we searched for occurrences of relevant keywords, including methane, gas, white gas, gas station, steam, white steam, leak, plume, and infrared. The frequency distribution is shown in Figure \ref{fig:freq}. The chart indicates that "gas" and "steam" are among the most frequently appearing terms. However, despite its higher frequency, prompts containing "gas" performed worse than those using "steam."

To further investigate this discrepancy, we generated word clouds from dataset entries containing "gas" and "steam" (Figure \ref{fig:wordcloud}). The word cloud for "gas" predominantly includes terms such as gas mask, gas station, oil, and gas fireplace—contexts that are semantically related to gas but do not visually resemble a gas leak. In contrast, the word cloud for "steam" is often associated with terms like steam locomotive and steam train, which visually feature steam being released from a chimney.

Additionally, because gas is generally invisible in RGB images—likely the primary modality used in the dataset—the model may struggle to associate the term "gas" with its visual appearance in inferred images. This suggests that the model’s underperformance on prompts containing "gas" is likely due to a mismatch between the term’s training data associations and its expected visual representation in real-world scenarios.

In our ablation study on different prompts, "white steam" and "white smoke" performed the best, whereas "white plume" exhibited the worst performance. We hypothesize that the superior performance of "white steam" and "white smoke" is due to their explicit description of both the substance (smoke or steam) and its color (white). In contrast, the poor performance of "white plume" is likely because "plume" is a relatively uncommon word.  

Notably, the prompts "white gas" and "gas leak" also performed poorly. We attribute this to the fact that, in the training data of vision-language models (VLMs), "gas" is often associated with "gas station," rather than referring solely to a gaseous substance. As a result, the model may tend to link "gas" to "gas station" or "gas stove," leading to suboptimal performance. Additionally, since gases are generally invisible in RGB images, and RGB is likely the primary modality in the training dataset, the model may struggle to associate the term "gas" with its visual characteristics in infrared imagery. This suggests that the poor performance of prompts containing "gas" is likely due to a mismatch between the term's associations in the training data and its expected visual representation in real-world scenarios.  

Another notable observation is that the long prompt, "white methane leak on black background in infrared image," achieved near-optimal performance, only slightly worse than the best-performing prompts. We hypothesize that while the VLM may not have a strong understanding of "methane," the explicit description of the black background and the infrared image modality provide sufficient context for the model to generate accurate outputs.

